Tool Demonstration: FSolidM for Designing Secure Ethereum Smart Contracts

Blockchain-based distributed computing platforms enable the trusted execution of computation - defined in the form of smart contracts - without trusted agents. Smart contracts are envisioned to have a variety of applications, ranging from financial to IoT asset tracking. Unfortunately, the development of smart contracts has proven to be extremely error prone. In practice, contracts are riddled with security vulnerabilities comprising a critical issue since bugs are by design non-fixable and contracts may handle financial assets of significant value. To facilitate the development of secure smart contracts, we have created the FSolidM framework, which allows developers to define contracts as finite state machines (FSMs) with rigorous and clear semantics. FSolidM provides an easy-to-use graphical editor for specifying FSMs, a code generator for creating Ethereum smart contracts, and a set of plugins that developers may add to their FSMs to enhance security and functionality.

==> accessControl.tex <==
\section{Implementation of the Access Control Plugin}
\label{sec:accessContrImpl}

%\subsubsection{Implementation}

Here, we describe the implementation of the access control plugin, which is introduced in Section~\ref{sec:accessContr}.

If the access control plugin is enabled, then
\begin{align*}
\lbl{Plugins} ~{+\!\!=} ~&\code{mapping(address => bool) private isAdmin;} \\
&\code{uint private numAdmins = 1;} \\
& \\
& \code{function } name \code{() \{} \\
& \ind \code{isAdmin[msg.sender] = true;} \\
%& \ind \code{numAdmins = 1;} \\
& \code{\}} \\
& \\
& \code{modifier onlyAdmin \{} \\
& \ind \code{require(isAdmin[msg.sender]);} \\
& \ind \code{\char`_;} \\
& \code{\}} \\
& \\
& \code{function addAdmin(address admin) onlyAdmin \{} \\
& \ind \code{require(!isAdmin[admin]);} \\
& \ind \code{isAdmin[admin] = true;} \\
& \ind \code{numAdmins += 1;} \\
& \code{\}} \\
& \\
& \code{function removeAdmin(address admin) onlyAdmin \{} \\
& \ind \code{require(isAdmin[admin]);} \\
& \ind \code{require(numAdmins > 1);} \\
& \ind \code{isAdmin[admin] = false;} \\
& \ind \code{numAdmins -= 1;} \\
& \code{\}}
\end{align*}
For transitions $t$ such that $\lbl{admin} \in t^{tags}$ (i.e., transitions that are tagged ``only admin'' by the developer), 
\begin{align*}
\lbl{TransitionPlugins}(t) ~{+\!\!=} ~&\code{onlyAdmin}
\end{align*}

==> numerical.tex <==
\subsection{Numerical Results on Computational Cost}
\label{sec:numerical}

Plugins not only enhance security but also increase the computational cost of transitions.
Since users must pay a relatively high price for computation performed on the public Ethereum platform, the computational cost of plugins is a critical question.
Here, we measure and compare the computational cost of transitions in our blind-auction contract without and with the locking and transition counter plugins.
We focus on these security feature plugins because they introduce overhead, while the design pattern plugins introduce useful functionality.

For this experiment, we use Solidity compiler version 0.4.17 with optimizations enabled.
In all cases, we quantify computational cost of a transition as the gas cost of an Ethereum transaction that invokes the function implementing the transition.\footnote{Gas measures the cost of executing computation on the Ethereum platform.}
The cost of deploying our smart contract was 504,672 gas without any plugins, 577,514 gas with locking plugin, 562,800 gas with transition counter plugin, and 637,518 gas with both plugins.\footnote{At the time of writing, this cost of deployment was well below \$1 (if the deployment does not need to be prioritized).}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=1.05\textwidth,
    height=0.5\textwidth,
    bar width=0.018\textwidth,
    ybar,
    ymin=0,
    ylabel={Transaction cost [gas]},
    legend pos=north east,
    symbolic x coords={{bid}, {cancelABB}, {unbid}, {close}, {reveal}, {finish}, {withdraw}},
    xtick=data,
    xticklabel style={font=\small\tt},
    ]
    \addplot coordinates { % without locking
        (bid, 58249)        
        (cancelABB, 42059)  
        (unbid, 19735)
        (close, 42162)
        (reveal, 65729)
        (finish, 27239)
        (withdraw, 20290)
    };
    \addlegendentry{without plugins};
    \addplot coordinates { % with locking
        (bid, 68917)        
        (cancelABB, 52727)
        (unbid, 30406)
        (close, 52830)
        (reveal, 76415)
        (finish, 37913)
        (withdraw, 30961)
    };
    \addlegendentry{with locking};
    \addplot coordinates { % with counter
        (bid, 63924)        
        (cancelABB, 47661)
        (unbid, 25406)
        (close, 47764)
        (reveal, 71390)
        (finish, 32891)
        (withdraw, 25961)
    };
    \addlegendentry{with counter};
    \addplot coordinates { % with both
        (bid, 74607)        
        (cancelABB, 58329)
        (unbid, 36074)
        (close, 58432)
        (reveal, 82067)
        (finish, 43559)
        (withdraw, 36629)
    };
    \addlegendentry{with both};
\end{axis}
\end{tikzpicture}
\caption{Transaction costs in gas without plugins (\textcolor{blue}{\bf blue}), with locking plugin (\textcolor{red}{\bf red}), with transition counter plugin (\textcolor{brown}{\bf brown}), and with both plugins (\textcolor{darkgray}{\bf dark gray}).}
\label{fig:transCosts}
\end{figure}

Figure~\ref{fig:transCosts} (and Table~\ref{tab:transCosts} in Appendix~\ref{sec:numericalTable}) shows the gas cost of each transition for all four combinations of the two plugins. 
We make two key observations.
First, \emph{computational overhead is almost constant} for both plugins and also for their combination.
For example, the computational overhead introduced by locking varies between 10,668 and 10,686 gas.
For the simplest transition, \texttt{unbid}, this constitutes a 54\%  increase in computational cost,
while for the most complex transition, \texttt{reveal}, the increase is 16\%.
Second, the \emph{computational overhead of the two plugins is additive}. The increase in computational cost for enabling locking, transition counter, and both are around 10,672 gas, 5,648 gas, and 16,319 gas, respectively.





==> numericalTable.tex <==
\section{Numerical Results on Computational Cost -- Table}
\label{sec:numericalTable}

Table~\ref{tab:transCosts} shows the gas cost of each transition for all four combinations of the \emph{locking} and \emph{transition counter} plugins.
Please see Section~\ref{sec:numerical} for a discussion of these results.

\begin{table}
\centering
\caption{Computational Cost of Transitions}
\label{tab:transCosts}
\setlength{\tabcolsep}{0.6em}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|r|r|r|r|}
\hline
Transition & \multicolumn{4}{c|}{Computational cost [gas]} \\
\cline{2-5}
 & without plugins & with locking & with transition counter & with both \\
\hline
\texttt{bid} & 58,249 & 68,917 & 63,924 & 74,607 \\
\texttt{cancelABB} & 42,059 & 52,727 & 47,661 & 58,329 \\
\texttt{unbid} & 19,735 & 30,406 & 25,406 & 36,074 \\
\texttt{close} & 42,162 & 52,830 & 47,764 & 58,432 \\
\texttt{reveal} & 65,729 & 76,415 & 71,390 & 82,067 \\
\texttt{finish} & 27,239 & 37,913 & 32,891 & 43,559 \\
\texttt{withdraw} & 20,290 & 30,961 & 25,961 & 36,629 \\
\hline
\end{tabular}
\end{table}
 

==> prelim.tex <==
%\section{Preliminaries}
%\label{sec:prelim}

%\subsection{Ethereum and Solidity}

\subsubsection{Common Vulnerabilities}
\label{sec:commonVuln}

\begin{itemize}
\item reentrancy
\item order of transactions
(``transaction-ordering dependence''~\cite{luu2016making} and ``unpredictable state''~\cite{atzei2017survey})
\item logical flaws
\Aron{This not very specific...}
\end{itemize}
\Aron{Cite papers!}

\begin{table}
\caption{Common Smart-Contract Vulnerabilities}
\centering
\begin{tabular}{|l|l|}
\hline
Vulnerability & Mitigation \\
\hline\hline
reentrancy & locking (Section~\ref{sec:locking}) \\
unpredictable state & transition counter (Section~\ref{sec:transCounter}) \\
logical flaws & access control (Section~\ref{sec:accessContr}), timed transitions (Section~\ref{sec:timedTrans}) \\
\hline
\end{tabular}
\end{table}

\Natassa{Maybe we could add a table here with a summary of the known vulnerabilities and say which ones we address with our implementation?}

==> related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Common Vulnerabilities and Design Patterns}
\label{sec:commonVuln} 

Multiple studies investigate and provide taxonomies for common security vulnerabilities and design patterns in Ethereum smart contracts.
In Table~\ref{tab:common}, we list the vulnerabilities that we address and the patterns that we implement in our framework using plugins.

\begin{table}
\setlength{\tabcolsep}{0.75em}
\renewcommand{\arraystretch}{1.2}
\caption{Common Smart-Contract Vulnerabilities and Design Patterns}
\label{tab:common}
\centering
\begin{tabular}{|l|l|l|}
\hline
Type & Common Name & FSolidM Plugin \\
\hline\hline
\multirow{3}{*}{Vulnerabilities} & reentrancy~\cite{luu2016making,atzei2017survey} & locking (Section~\ref{sec:locking}) \\ 
\cline{2-3}
& transaction ordering~\cite{luu2016making} & transition counter (Section~\ref{sec:transCounter}) \\
& a.k.a. unpredictable state~\cite{atzei2017survey} & \\
\hline
\multirow{2}{*}{Patterns} & time constraint~\cite{bartoletti2017empirical} & timed transitions (Section~\ref{sec:timedTrans}) \\
\cline{2-3}
& authorization~\cite{bartoletti2017empirical} & access control (Section~\ref{sec:accessContr}) \\
\hline
\end{tabular}
\end{table}

Atzei et al.\ provide a detailed taxonomy of security vulnerabilities in Ethereum smart contracts, identifying twelve distinct types~\cite{atzei2017survey}.
For nine vulnerability types, they show how an attacker could exploit the vulnerability to steal assets or to cause damage. 
Luu et al.\ discuss four of these vulnerability types in more detail, proposing various techniques for mitigating them (see Section~\ref{sec:verification})~\cite{luu2016making}.
In this paper, we focus on two types of these common vulnerabilities:
\begin{compactitem}
\item Reentrancy Vulnerability: Reentrancy is one of the most well-known vulnerabilities, which was also exploited in the infamous ``The DAO'' attack.
In Ethereum, when a contract calls a function in another contract, the caller has to wait for the call to finish. 
This allows the callee, who may be malicious, to take advantage of the intermediate state in which the caller is, e.g., by invoking a function in the caller.
\item Transaction-Ordering Dependence:
If multiple users invoke functions in the same contract, the order in which these calls are executed cannot predicted.
Consequently, the users have uncertain knowledge of the state in which the contract will be when their individual calls are executed. 
\end{compactitem}

%Focusing on the development of smart contracts,
Bartoletti and Pompianu 
identify nine common design patterns in Ethereum smart contracts, %, such as authorization and time constraints, 
and measure how many contracts use these patterns in practice~\cite{bartoletti2017empirical}.
Their results show that the two most common patterns are \emph{authorization} and \emph{time constraint}, which are used in 61\% and 33\% of all contracts, respectively. 
The also provide a taxonomy of Bitcoin and Ethereum contracts, dividing them into five categories based on their application domain.
Based on their categorization, they find that the most common Ethereum contracts deployed in practice are financial, notary, and games. 

% OLD VERSION
\begin{comment}
\subsection{Common Vulnerabilities and Design Patterns}
\label{sec:commonVuln} 

Multiple studies investigate and classify common security vulnerabilities in smart contracts.
% Making Smart Contracts Smarter
Luu et al.\ identify four classes of typical vulnerabilities in Ethereum smart contracts~\cite{luu2016making}.
\begin{compactitem}
\item Reentrancy Vulnerability: Reentrancy is one of the most well-known vulnerabilities, which was also exploited in the infamous ``The DAO'' attack.
In Ethereum, when a contract calls a function in another contract, the caller has to wait for the call to finish. 
This allows the callee, who may be malicious, to take advantage of the intermediate state in which the caller is, e.g., by invoking a function in the caller.
\item Transaction-Ordering Dependence:
If multiple users invoke functions in the same contract, the order in which these calls are executed cannot predicted.
Consequently, the users have uncertain knowledge of the state in which the contract will be when their individual calls are executed. 
\item Timestamp Dependence:
In Ethereum, a malicious participant may be able to alter the clock used in the execution of smart contracts by up to 900 seconds.\footnote{A miner can choose the timestamp of a new block maliciously; however, other miners will accept the block only if its timestamp is within a certain range of their clocks.}
As result, contracts whose correctness depends on the accuracy of the clock may be vulnerable.
\item Mishandled Exceptions:
Depending on how a function is called, an exception in the callee may or may not be propagated to the caller.
Due to the inconsistency of the propagation policy, developers can easily forget to properly handle exceptions in callee contracts.
\end{compactitem}
% A Survey of Attacks on Ethereum Smart Contracts (SoK)
Atzei et al.\ provide a more detailed taxonomy of security vulnerabilities in Ethereum smart contracts, identifying twelve distinct classes.
For nine of these classes, they show how an attacker could exploit the vulnerability to steal assets or to cause damage~\cite{atzei2017survey}. \Natassa{For me it is not clear how security vulnerabilities and security bugs are different. If they are the same, or at least similar, then we should make the connection with the previously mentioned security bugs.}
\Aron{I think that we can use ``vulnerabilities'' and ``security bugs'' interchangeably.}

% An empirical analysis of smart contracts: platforms, applications, and design patterns
Focusing on the development of smart contracts,
Bartoletti and Pompianu 
analyze Bitcoin and Ethereum contracts deployed in practice and provide a taxonomy of contracts~\cite{bartoletti2017empirical}.
They also identify nine common design patterns, such as time constraints and authorization, and quantify their usage. \Natassa{I think we need to mention how our work is related or mitigates the identified security bugs/vulnerabilities and whether we are using any of the identified design patterns (Luu et al., Atzei et al., Bartoletti et al.). Currently, Table 1 presents the correlation with two of the security bugs identified by Luu et al. but we need to do the same for the other papers. I understand that we can not actually tackle all the vulnerabilities explored with our approach. But what we can say is that this paper is a proof of concept in which we picked some of the most important identified vulnerabilities. Future work includes adding security patterns for the other vulnerabilities.}

\begin{table}
\caption{Common Smart-Contract Vulnerabilities}
\centering
\begin{tabular}{|p{2.95cm}|p{8.5cm}|}
\hline
Vulnerability & Mitigation \\
\hline\hline
reentrancy & locking (Section~\ref{sec:locking}) \\ 
\hline
transaction ordering 
(unpredictable state) & transition counter (Section~\ref{sec:transCounter}) \\
\hline
logical flaws & access control (Section~\ref{sec:accessContr}), timed transitions (Section~\ref{sec:timedTrans}) \\
\hline
\end{tabular}
\end{table}
\Natassa{where is Table 1 referenced in the text?}
\end{comment}

\subsection{Verification and Automated Vulnerability Discovery}
\label{sec:verification}

Multiple research efforts attempt to identify and fix these vulnerabilities through verification and vulnerability discovery.
% Formal Verification of Deed Contract in Ethereum Name Service
For example, Hirai first performs a formal verification of a smart contract that is used by the Ethereum Name Service~\cite{hirai2016formal}.\footnote{The Ethereum Name Service is a decentralized service, built on smart contracts, for addressing resources using human-readable names.}
However, this verification proves only one particular property and it involves relatively large amount of manual analysis.
In later work, Hirai defines the complete instruction set of the Ethereum Virtual Machine in Lem, a language that can be compiled for interactive theorem provers~\cite{hirai2017defining}.
Using this definition, certain safety properties can be proven for existing contracts.

% Short Paper: Formal Verification of Smart Contracts (2016)
Bhargavan et al.\ outline a framework for analyzing and verifying the safety and correctness of Ethereum smart contracts~\cite{bhargavan2016short}.
The framework is built on tools for translating Solidity and Ethereum Virtual Machine bytecode contracts into $F^*$, a functional programming language aimed
at program verification.
Using the~$F^*$ representations, the framework can verify the correctness of the Solidity-to-bytecode compilation as well as detect certain vulnerable patterns. % safety and functional-correctness properties of the contracts. 

% Making Smart Contracts Smarter
Luu et al.\ propose two approaches for mitigating common vulnerabilities in smart contracts~\cite{luu2016making}.
First, they recommend changes to the execution semantics of Ethereum, which eliminate vulnerabilities from the four classes that they identify in their paper.
However, these changes would need to be adopted by all Ethereum clients. 
As a solution that does not require changing Ethereum, they provide a tool called \textsc{Oyente}, which can analyze smart contracts and detect certain security vulnerabilities.





%%% UNORGANIZED

\begin{comment}

% Short Paper: Formal Verification of Smart Contracts (2016)
% https://www.cs.umd.edu/~aseem/solidetherplas.pdf
Bhargavan et al.\ outline a framework for analyzing and verifying the safety and correctness of Ethereum smart contracts~\cite{bhargavan2016short}.
The framework is built on tools for translating Solidity and Ethereum Virtual Machine bytecode contracts into $F^*$, a functional programming language aimed
at program verification.
Using the~$F^*$ representations, the framework can verify the correctness of the Solidity compilation as well as certain safety and functional-correctness properties of the contracts.

% Making Smart Contracts Smarter
Luu et al.\ identify classes of typical security bugs in Ethereum smart contracts and propose two approaches for mitigating these vulnerabilities~\cite{luu2016making}.
First, they recommend changes to the execution semantics of Ethereum, which eliminate the vulnerabilities identified in the paper; however, these changes would have to be adopted by all Ethereum clients. 
As a solution that does not require changing Ethereum, they provide a tool called \textsc{Oyente}, which can analyze smart contracts and detect certain security vulnerabilities.

% A Survey of Attacks on Ethereum Smart Contracts (SoK)
Atzei et al.\ provide a taxonomy of security vulnerabilities in Ethereum smart contracts and show how attackers could exploit them to steal assets or cause damage~\cite{atzei2017survey}.

% An empirical analysis of smart contracts: platforms, applications, and design patterns
Bartoletti and Pompianu 
analyze Bitcoin and Ethereum contracts deployed in practice and provide a taxonomy of contracts~\cite{bartoletti2017empirical}.
They also identify nine common design patterns and quantify their usage.

% Formal Verification of Deed Contract in Ethereum Name Service
Hirai performs a formal verification of a smart contract that is used by the Ethereum Name Service~\cite{hirai2016formal}.
\footnote{The Ethereum Name Service is a decentralized service, built on smart contracts, for addressing resources using human-readable names.}
However, the verification proves only one particular property and it involves relatively large amount of manual analysis.

\end{comment}


==> rockpaperscissors.tex <==
\subsection{Rock-Paper-Scissors}

Consider a contract modeling an electronic rock-paper-scissors game.
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Play}, in which the two participants may submit their blinded choices (i.e., submit the hash values of their choices) if they make deposits;
\item \texttt{Reveal}, in which the participants reveal their choices; 
\item \texttt{Finished}, in which the winning participant may withdraw the deposits;
\item \texttt{Canceled}, in which the cooperating participant may withdraw the deposits (contract transitions to this state if the other participant did not submit a choice or did not reveal it in time).
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{choose} (from state \texttt{Play} to state \texttt{Play}):
submits a blinded choice and makes a deposit (tagged $\lbl{payable}$);
\item \texttt{close} (from state \texttt{Play} to state \texttt{Reveal}): starts the reveal phase if both participants submitted a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{cancelPlay} (from state \texttt{Play} to state \texttt{Canceled}): cancels the game if one of the participants did not submit a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{reveal} (from state \texttt{Reveal} to state \texttt{Reveal}): reveals a blinded choice;
\item \texttt{finish} (from state \texttt{Reveal} to state \texttt{Finished}): finishes the game and declares winner (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawFinished} (from state \texttt{Finished} to state \texttt{Finished}): withdraws the deposits
 (may be called only by the winning participant);
\item \texttt{cancelReveal} (from state \texttt{Reveal} to state \texttt{Canceled}): cancels the game if one of the participants did not reveal its blinded choice
 (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawCanceled} (from state \texttt{Canceled} to state \texttt{Canceled}): withdraws the deposits
 (may be called only by the cooperating participant).
\end{itemize}

==> voting.tex <==
\subsection{Voting}

Consider a voting contract, in which an administrator can assign voting rights to participants (identified using their Ethereum addresses), who may cast one vote each. 
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Setup}, in which administrators can add or remove participants, as well as add or remove options on which the participant may vote;
\item \texttt{Casting}, in which participants may cast their votes; 
\item \texttt{Closed}, in which the option with the most votes is declared winner;
\item \texttt{Canceled}, in which no winning option is selected.
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{addParticipant}, \texttt{removeParticipant} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting participant (transition tagged $\lbl{admin}$);
\item \texttt{addOption}, \texttt{removeOption} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting option (transition tagged $\lbl{admin}$);
\item \texttt{open} (from state \texttt{Setup} to state \texttt{Casting}):
begins the voting process (timed transition);
\item \texttt{cast} (from state \texttt{Casting} to state \texttt{Casting}):
casts a vote on an option (may be called only by a participant);
\item \texttt{close} (from state \texttt{Casting} to state \texttt{Closed}):
closes the voting process and declares a winning option (timed transition, with a guard on the number of votes casted);
\item \texttt{cancel} (from state \texttt{Casting} to state \texttt{Canceled}):
cancels the voting process (timed transition, with a guard on the number of votes casted).
\end{itemize}
